Adaptive BEM for elliptic PDE systems, part II: Isogeometric analysis with hierarchical B-splines for weakly-singular integral equations

We formulate and analyze an adaptive algorithm for isogeometric analysis with hierarchical B-splines for weakly-singular boundary integral equations. We prove that the employed weighted-residual error estimator is reliable and converges at optimal algebraic rate. Numerical experiments with isogeometric boundary elements for the 3D Poisson problem confirm the theoretical results, which also cover general elliptic systems like linear elasticity.

==> 05_proof_high.tex <==
% !TEX encoding = MacOSRoman
% !TEX root = igabem3d.tex

%\section{Proof of Theorem~\ref{thm:main bem}}
%\label{sec:proof bem}
%This section is devoted to the proof of Theorem~\ref{thm:main bem}, i.e., to the verification of the mesh properties \eqref{M:patch bem}--\eqref{M:semi bem}, the refinement properties \eqref{R:sons bem}--\eqref{R:overlay bem}, and the boundary element space properties \eqref{S:inverse bem}--\eqref{S:stab bem}.





